Head-mouse: A simple cursor controller based on optical measurement of head tilt

This paper describes a wearable wireless mouse-cursor controller that optically tracks the degree of tilt of the user's head to move the mouse relative distances and therefore the degrees of tilt. The raw data can be processed locally on the wearable device before wirelessly transmitting the mouse-movement reports over Bluetooth Low Energy (BLE) protocol to the host computer; but for exploration of algorithms, the raw data can also be processed on the host. The use of standard Human-Interface Device (HID) profile enables plug-and-play of the proposed mouse device on modern computers without requiring separate driver installation. It can be used in two different modes to move the cursor, the joystick mode and the direct mapped mode. Experimental results show that this head-controlled mouse to be intuitive and effective in operating the mouse cursor with fine-grained control of the cursor even by untrained users.

==> approach.tex <==
% approach.tex

\section{Technical Approach}
\label{sec:approach}

The system uses two sets of IR-based sensors to measure relative distance
between the bottom of the chin and the deck on which the sensors are placed.
Each sensor consists of an IR transmitter and a receiver. The photo diode
receiver is sensitive enough to detect IR reflection from the surface facing the
sensor. 
\begin{cmtPai}
(9/1/2017) I think you are repeating what was written earlier already. What
you need is a topic sentence at the beginning of the paragraph, and the rest
of the paragraph should stay within the scope of that topic sentence.
\end{cmtPai}

In resting position, two sensors approximately receive the same amount
of IR signal due to symmetry. Tilting down the user's head brings both sensors
closer to the surface of reflection, resulting in a stronger signal. Likewise,
tilting up the head weakens the reflection received by both sensors due to the
longer distance.  


When the head is rolled to the right, the left sensor sees a
weak reflection from the left side of the chin, but the right sensor sees little
change in the reflection since the chin is still above the receiver. Thus, a
weak signal on the left sensor and a strong signal on the right sensor indicates
a cursor movement to right.  The same is applied to left rolling.

\FIG{system}(c) shows the signal values for different movements of pitching
forward and backward 
\begin{cmtPai}
(9/1/2017) pitch is more like tilting up/down rotation, right? forward/back
does not sound like rotation but more like linear motion.
\end{cmtPai}
and yawing to the left and right. The yawing movement is
translated to a horizontal cursor movement on the 2-D screen while pitching
backward-and-forward is interpreted as vertical up-and-down cursor movements.
\begin{cmtPai}
(9/1/2017) again, I think the reader has figured this out by now, so no need
to dwell on this, but you need to show a more systematic, either algorithmic
or mathematical way to perform this mapping.
\end{cmtPai}

Photodiodes then outputs the recorded reflection
signal as a voltage which digitized by the ADC on the micro controller.
\begin{cmtPai}
(9/1/2017) the rest of this paragraph is repetitive. I'd say delete and merge
this section with the method section directly.
\end{cmtPai}
Next, the signals go through a series of processing on the micro controller to
map the head movement to cursor movement. Two different modes of joystick and
direct mapping are implemented. The details of these two regimes are brought in
\SEC{sec:results}.




==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\begin{cmtPai}
(8/30/2017) I merged the writeup of this implementation section into the
previous one, so I think this file can be removed.
\end{cmtPai}



==> related.tex <==
\section{Related Work}
\label{sec:related}
\begin{cmtPai}
	(8/30/2017) You need a related work section to discuss alternative options,
	the pros and cons, and issues.
\begin{itemize}
\item camera based: eye tracker, face tracker
\item tongue control: pro = accurate control, not require head; con =
	complicated setup?
\item EMG (muscle tension): pro = sensitive and accurate? con = uncomfortable?
\item EEG (brain wave): pro = pick up many signals? con = complicated, bulky?
\item optical -- is there any other system? pro = low cost, simple mechanism,
	low computational complexity, etc; con = potential noise from stray light,
	including ambient light?
\end{itemize}
\end{cmtPai}
